The effect of tides on the Sculptor dwarf spheroidal galaxy

Dwarf spheroidal galaxies (dSphs) appear to be some of the most dark matter dominated objects in the Universe. Their dynamical masses are commonly derived using the kinematics of stars under the assumption of equilibrium. However, these objects are satellites of massive galaxies (e.g.\ the Milky Way) and thus can be influenced by their tidal fields. We investigate the implication of the assumption of equilibrium focusing on the Sculptor dSph by means of ad-hoc $N$-body simulations tuned to reproduce the observed properties of Sculptor following the evolution along some observationally motivated orbits in the Milky Way gravitational field. For this purpose, we used state-of-the-art spectroscopic and photometric samples of Sculptor's stars. We found that the stellar component of the simulated object is not directly influenced by the tidal field, while $\approx 30\%-60\%$ the mass of the more diffuse DM halo is stripped. We conclude that, considering the most recent estimate of the Sculptor proper motion, the system is not affected by the tides and the stellar kinematics represents a robust tracer of the internal dynamics. In the simulations that match the observed properties of Sculptor, the present-day dark-to-luminous mass ratio is $\approx 6$ within the stellar half-light radius ($\approx0.3$ kpc) and $>50$ within the maximum radius of the analysed dataset ($\approx1.5^\circ\approx2$ kpc).

==> include/Discussion/Discussion_old.tex <==
\section{Discussion and conclusions} \label{sec:dicussion}



In this work, we used ad-hoc $N$-body simulations to analyse the dynamical evolution of the Sculptor dSph in the tidal field of the MW.  
The dynamical models of the satellite and its backward orbits have been based on state-of-the-art observational data (see Sec.\ \ref{sec:theScl}).
Our final simulations are able to nicely reproduce the current position and velocities of Sculptor as well as the observed angle-averaged los surface density and velocity dispersion profile.  
The results of this work (Sec.\ \ref{sec:fresults})  indicate that even considering one of the most eccentric orbit allowed by the data uncertainties  (primarily on proper motion but also on other quantities, see Sec.\ \ref{sec:orbinv}) the direct effects of tides on the baryonic content of the satellite are negligible, in particular, no significant and detectable tidal tails are developed. 
Even if not directly affected by tides, the stellar component of the satellite show a certain degree of evolution because of the response to the significant mass loss experienced by the more extended DM halo. In particular,   the half-light radius increases  and the los velocity dispersion decreases. 
However, in the last 2 Gyr the evolution proceeds very slowly, the properties of the baryonic component changes less than about 5\% and the satellite in the last snapshots is close to equilibrium in its own gravitational potential. These results suggest that the assumption of dynamical equilibrium can be safely used to estimate the dynamical mass of Sculptor (Sec.\ \ref{sec:mockfit}), moreover the lack of stellar tidal tails in the simulation indicate that we can consider the existing kinematic samples free from contamination by tidally stripped stars.
These results are similar to what obtained by \cite{Fornax15} for Fornax dSph and they are compatible with the results of \cite{penarrubia09}.

The lack of development of stellar tidal tails in both the FH18 and EH18 simulations  suggests that the Plummer-like profile observed in Sculptor is likely an intrinsic property of the system and it is not caused by a  transformation of a primordial King profile as can be the case of objects heavily affected by tides \cite{penarrubia09}.  

Recently \cite{hammer1} pointed out that the gravitational acceleration due to the MW is heavily affecting the  los velocity dispersion of satellites. In particular, for Sculptor and other classical dSphs this effect alone could explain the observed high magnitude los  velocity dispersion.
Since this is a purely gravitational effect, its imprint should be present in our simulations. 
However, we found that in all our simulations either including an extended DM halo (Sec.\ \ref{sec:evres}) or assuming a mass-follows-light model (Sec.\ \ref{sec:mfl}) the evolution of the los velocity dispersion profile within the observed range is driven by the mass loss of the DM halo and/or the property of the baryonic component.  
This is particularly evident in the mass-follows-light models where the lack of an extended DM halo should make the effect of the MW acceleration postulated by \cite{hammer1} clearly evident.
The  right-hand panels of  Fig.\ \ref{fig:mfl} show that at the half-light radius, where the satellite is not affected by tides, the los velocity dispersion is totally dependent on the distribution of matter inside the galaxy  (both on shape and magnitude) while the \cite{hammer1} model predicts a  higher\footnote{This value is obtained  using the \JP MW potential model in the  Eq.\ B16 of  \cite{hammer1}} $\sigma_\te{los} \approx 12 \ \kms$.
Therefore, we conclude that the effect described by \cite{hammer1} is not important for Sculptor and the observed high-magnitude and flat los velocity dispersion profile is a genuine signature of the presence of an extended DM halo surrounding the baryonic component.
In this context,the simulations that successfully reproduce Sculptor's observables have  dark-to-luminous mass ratio  5.9 (FH18$_{14}$) and 5.8 (EH18$_{17}$)  within the projected stellar half-mass radius (283 pc in  FH18$_{14}$ and  271 pc in EH18$_{17}$)   and 61.5 (FH18$_{14}$) and  52.9 (EH18$_{17}$)  within the projected $R_*=1.5^\circ$ radius (2.25 kpc in  FH18$_{14}$ and 2.16 kpc in EH18$_{17}$). 

The results of this work are based on a number of working assumption. Most of them are simplifications that we tuned with the idea to maximise the possible tidal effects. 
First of all, we used a fixed external potential considering a \vir{fully grown} MW for the entire $\approx 7 \ \te{Gyr}$ of the orbital evolution. The used potential is a simple analytic model \JP that represent a \vir{heavy} MW ($M_{200}>2\times10^{12} \ \msun$, see Sec.\ \ref{sec:orbital:mw}). 
Although this model does not represent the state of the art of the dynamical modelling of the MW and it does not take into account the hierarchical mass evolution of the Galaxy, it maximises the influence of tides on Sculptor. Therefore, our results are robust given that the if the tidal effects are not important in the analysed case it is likely that this holds even considering more sophisticated and time-dependent MW potential models. 
Another fundamental assumption is that we consider only spherical and isotropic satellite models.  

-isotropia e forma.
-core.
-implications.

Our satellite model is isotropic and spherical 



Discuss hammer
